The Raspberry Pi Auto-aligner: Machine Learning for Automated Alignment of Laser Beams

We present a novel solution to automated beam alignment optimization. This device is based on a Raspberry Pi computer, stepper motors, commercial optomechanics and electronic devices, and the open source machine learning algorithm M-LOOP. We provide schematic drawings for the custom hardware necessary to operate the device and discuss diagnostic techniques to determine the performance. The beam auto-aligning device has been used to improve the alignment of a laser beam into a single-mode optical fiber from manually optimized fiber alignment with an iteration time of typically 20~minutes. We present example data of one such measurement to illustrate device performance.

==> NOTES.tex <==
%Several types of ML algorithms such as genetic algorithms (GAs) and deep neural networks (DNNs) have been used for optics experiments \cite{Kutz18}. However the simplest to use software, which is designed to be easily interfaced with an experiment, is M-LOOP \cite{Hush16}.

%The code for the deep learning architecture, created by Baumeister \emph{et al.} \cite{Kutz18}, can be found at: \url{https://github.com/thombau/UW\_Seattle\_1}.

%Shift registers (SRs) were incorporated into the experiment, giving the potential for control of a larger number of experimental parameters. Used in serial-in-parallel-out (SIPO) mode, SRs can amplify the limited number of general-purpose input-output (GPIO) pins on the Pi, allowing simultaneous control of any number of parameters with almost zero time-lag. A SR is also necessary to prevent the recommended maximum current output of the Pi being surpassed when using four motors. A schematic of the operation of a shift register is shown in Fig. A.1. The 74HC595 shift register is capable of operating two bipolar stepper motors, therefore two shift registers must be connected in series (daisy-chained) to operate four such motors. To
%operate an individual motor requires four-bit instructions and therefore operating four in parallel requires sixteen-bit instructions. The code used to operate the motors can be found in Appendix A Section 2, and a schematic of the electronic components in shown in Fig. 4


%An analogue-to-digital converter (ADC), the 16-bit ADS1115 ADC, is used to convert the analogue output of a photodiode (PD) to the digital signal required by the Raspberry Pi.

%NEMA stepper motors are commonly used in computer numerical control (CNC) machines and are readily available.


%Mirror mounts have knobs which convert rotation into angular displacement of the mirrors. A motor is attached to knob controlling the pitch of the mirror and another is attached to the knob controlling the yaw. A combination of pitch and yaw sets the orientation of the mirror. Stepper motors were chosen because they are inexpensive and easy to control, requiring less-complicated electronics than closed-loop motors. Initially 28BYJ-48 stepper motors were used, driven by ULN2003 boards. These motors suffered from significant backlash which resulted in a noticeable amount of lost motion.
%The motors we use are 28BYJ-48 5V Stepper Motors with ULN2003 driver boards. 
%They also have a low maximum torque and would frequently stall when coupled to the mirror mounts. NEMA-17 stepper motors (driven by L298N driver boards) were chosen to replace the 28BYJ-48 as they have higher torque and negligible backlash. NEMA stepper motors are commonly used in computer numerical control (CNC) machines, and were readily available at the beginning of this project. Two mirrors are required to fully control the alignment of a laser, requiring four motors.

%A coupler is necessary to connect the motor shaft to the mirror mount, and must be able to transfer the rotation of the motor to the mirror knob with as little lost motion as possible. Couplers were initially 3D-printed in plastic, allowing for rapid prototyping, however these degraded and morphed over time due to the force exerted by the motor and were eventually unable to transfer rotation to the mirror knob. Subsequent designs were machined in-house using steel.

%``To use this device, the only requirements are a suitable power supply (8 - 12~V DC, capable of supplying > 2 A), a computer monitor attached to the High-Definition Multimedia Interface (HDMI) port of the Raspberry Pi, and a mouse and keyboard attached via universal serial bus (USB). All processing is done on the Raspberry Pi. A USB memory stick or similar can be used to extract the gathered data. All custom-made components have relatively simple form, amenable to manufacture in any reasonable equipped workshop."

Due to a software driver incompatibility, the Raspberry Pi does not readily connect to either the power-meter (ThorLabs PM100D) or the photon-counter (Excelitas SPCM-AQRH Single Photon Counting Module in combination with a SensL HRM-TDC High Resolution Time-to-Digital Converter Module). To remedy this a desktop computer is implemented as an intermediary. Python sockets connect the desktop computer and the Pi: the computer (server) sends power-meter/photon-counter readings to the Pi (client) on request. The Pi and the computer can be connected wirelessly, although we did not implement this as we had a conveniently located ethernet port for a wired connection.

Due to the restricted number of GPIO pins on the Raspberry Pi, it is necessary to use shift registers in conjunction with the Raspberry Pi to increase the number of output ports. Shift registers are capable of controlling an arbitrary number of drivers/motors with almost zero time-lag. The 74HC595 shift register is used in this work as it is able to operate two bipolar stepper motors. To operate four motors, as is necessary for our beam auto-aligner, two shift registers are connected in series.

%@ARTICLE{Burt19,
%author = "Burt, D. R. and Rasmussen, C. E., and Van Der Wilk, M.",
%year = "2019",
%title = "Rates of convergence for
%sparse variational Gaussian process regression",
%journal = "ArXiv",
%url = "http://arxiv.org/abs/1903.03571",
%}
%@misc{burt2019rates,
 %   title={Rates of Convergence for Sparse Variational Gaussian Process Regression},
  %  author={David R. Burt and Carl E. Rasmussen and Mark van der Wilk},
   % year={2019},
    %eprint={1903.03571},
    %archivePrefix={arXiv},
    %primaryClass={stat.ML}

%}@article{Whiting_2017,
   title={Single-Photon Interference due to Motion in an Atomic Collective Excitation},
   volume={118},
   ISSN={1079-7114},
   url={http://dx.doi.org/10.1103/PhysRevLett.118.253601},
   DOI={10.1103/physrevlett.118.253601},
   number={25},
   journal={Physical Review Letters},
   publisher={American Physical Society (APS)},
   author={Whiting, D. J. and Šibalić, N. and Keaveney, J. and Adams, C. S. and Hughes, I. G.},
   year={2017},
   month={Jun}
}
%%%%%%%%%%% Thorlabs Table %%%%%%%%%%%
\begin{table}[h]
\centering
\caption[Features - Thorlabs Fiber-Control]{A summary of the main features of the Thorlabs Fiber-Control device.} 
\begin{tabular}{ p{150pt} | p{300pt} }

\large \textbf{Feature} & \large \textbf{Description} \\
 \hline
 Beam-alignment & Closed-loop feedback. \\
%\hline
 Angular Resolution & Piezos allow \SI{0.5}{\micro rad} resolution. Includes coarse-adjustment knobs.\\
%\hline
  Footprint & Controller: 121 mm x 60 mm x 47 mm.  Piezo-mounts have wires connected. \\
 % \hline 
  Price & Two-mirror-control: \pounds 3791.20 \\
 % \hline
  Software & Gradient-search - optical fiber is moved in a circle and a `power gradient search'  is performed.
\end{tabular}
\label{tab:Thorlabs}
\end{table}

%%%%%%%%%%% My Expt Setup Table %%%%%%%%%%%
\begin{table}[H]
\centering
\caption[Features - This experimental setup]{A summary of the main features of the experimental setup built in this project.} 
\begin{tabular}{ p{150pt} | p{300pt} }

\large \textbf{Feature} & \large \textbf{Description} \\
 \hline
 Type of alignment & (Potentially continuous) fiber--free-space alignment, open-loop feedback \\
%\hline
 Angular Resolution & Limited by step-size of motor, e.g. 0.9$^{\circ}$ using the 17HD48002H-22B stepper motor. \\
%\hline
  Footprint & Motor-Holder-Coupler system: 83 mm x 100 mm x 125 mm excluding footprint of the electronics.\\
%  \hline 
  Price & Dominated by Raspberry Pi and motors. RaspberryPi - \pounds 65.00, Motors (5) - \pounds 35.00.\\
%  \hline
  Software & Machine Learning - Gaussian Process
\end{tabular}
\label{tab:MySetup}
\end{table}

\begin{table}[tbh!]
\centering
\caption[Wiring - Raspberry Pi to Analog-to-Digital Converter]{The wiring from the Raspberry Pi to the Analog-to-Digital Converter} 
\begin{tabular}{ c | c | c }
\large \textbf{RPI Pins} & \large \textbf{ADS1115 ADC} & \large \textbf{Meaning}\\
 \hline
1 (3V3) & VDD  & Power\\
6 (GND) & GND  & Ground\\
3 (SDA3) & SDA  & Serial Data\\
5 (SCL3) & SCL  & Serial Clock \\
\end{tabular}
\label{tab:Pi to ADC}
\end{table}

\section{\label{sec:ADC}Reading from an ADC}

The analog-to-digital converter used in this work is the ADS1115 by Adafruit, who have written pre-made libraries to read data from their chips. To communicate with the chip it is necessary to download the library `Adafruit-CircuitPython-ADS1x15' from their GitHub, and add the library to the path.
\begin{python}
import sys
sys.path.append('/path/to/
Adafruit_CircuitPython_ADS1x15')

import adafruit_ads1x15.ads1115 as ADS
from adafruit_ads1x15.analog_in import AnalogIn
\end{python}

One can then read voltages from the ADC using
\begin{python}
i2c = busio.I2C(board.SCL, board.SDA) 
ads = ADS.ADS1115(i2c) 
channel = 0 # Can be changed-see datasheet
chan = AnalogIn(ads, channel)

def takeReading(n):
    allmV = [1000*chan.voltage for i in range(n)]
    avg = np.average(allmV) ; sterr=np.std(allmV)/len(allmV)**0.5
    return avg, sterr
\end{python}

It is possible the Adafruit library has deprecated since the completion of this project, however, there are alternative methods of communicating with the ADC, including using the SPI serial peripheral interface (see Figure \ref{fig:RPi_Pinout} for more details on implementing I2C and SPI communication using the Pi).

\begin{python}
import spidev
spi = spidev.SpiDev()

def readPhotoDiode(channel):
    spi.open(0,0) #Bus 0, Device 0
    spi.max_speed_hz = 5000  
    # Bus speed - see datasheet - 200 kHz at 5V
    raw_data = spi.xfer2([1,(8+channel)<<4,0]) 
    return_data = ((raw_data[1] & 3)<<8) +
    raw_data[2]
    mV = (float(return_data)*3300.)/1023 
    # return integer < 1024 given Pi voltage
    of 3.3 V 
    return round(mV,3)
    spi.close()
    # Use channel = 0 in the argument \textcolor{green}{not completely necessary}
\end{python}

Refer to the ADS1115 datasheet which specifies which bits of data read from the chip are useful and which are not, which should explain the `raw-data' and `return-data' lines above.

\section{Operating Shift Registers} \label{sec:operating_shift_registers}

Shift registers are capable of controlling an arbitrary number of drivers/motors with almost zero time-lag. The 74HC595 shift register is recommended to use for motors described in this work as it is able to operate two bipolar stepper motors. These shift registers work by accepting bits of information one at a time and transferring them to the storage register. One the register is full, the bits are then pushed to the output pins. Bits of information come in the form of HIGH or LOW square voltage pulses from the Pi. \\

It is necessary to `pulse' the shift register clock pin (SRCLK) in order to transfer one bit on each rising edge of the pulse. This is done by setting it to high voltage to allow one bit to be transferred to storage, then low voltage again to repeat the cycle. Once the storage register is full, the `latch' pin, or storage-register clock pin (RCLK) must be pulsed in the same way to allow the data to be pushed to the outputs. This is achieved using the following functions.

\begin{figure}[tbh!]
\centering
\includegraphics[width=0.7\textwidth]{figures/ShiftReigster-cropped.pdf} 
\caption[Shift Register Schematic]{Schematic shows the operation of  four-bit shift register chip. Firstly, bits are transferred to the storage register on the rising edge of the shift register clock signal. Once the storage register is full, bits are pushed to the output pins (Q0-3) on the rising edge of the storage register clock signal. The chip used in this project was an eight-bit shift register.}
\label{fig:shiftRegister}
\end{figure} 


\begin{python}
import RPi.GPIO as GPIO 

delay = 0.001
def pulseClock():
    GPIO.output(CLK, 1)
    time.sleep(delay)
    GPIO.output(CLK, 0)
    return
    
def pulseLatch():
    GPIO.output(LATCH,1)
    time.sleep(delay)
    GPIO.output(LATCH,0)
    return
\end{python}
The GPIO module controls the output voltages to the Pi's General-Purpose Input/Output pins, which can be set to HIGH (1) or LOW (0).\\

Bipolar stepper motors such as those used in this project require four bits of information to control each phase within the motor.
By sending a high voltage to one phase and low to all the others ([1,0,0,0]), then by repeating this for each phase in turn ([0,1,0,0], [0,0,1,0]...), continuous rotation of the motor shaft is achieved.\\

To control four motors, two eight-bit shift registers must be connected together, with the `data-out' pin (Q7') of the first being connected to the `data-in' pin of the second (DS).
This allows sixteen bits to be stored serially and output in parallel, i.e. in Serial-In-Parallel-Out (SIPO) mode. 
To control each motor at will and choose a clockwise or anticlockwise direction, these sixteen-bit `instructions' must be able to be chosen in the correct order.
\begin{python}
all_instructions =  []
states = [[1,0,0,0], [0,1,0,0], [0,0,1,0], [0,0,0,1]] 
position = np.arange(0,16,1)
x = np.zeros(16) 
instructions_motor_1 = []
for s in range(len(states)): #i.e. index over each set of instructions
    for i,j in zip(position[0:4], states[s]):
        x[i] = j
    instructions_motor_1.append(list(x))
all_instructions.append(instructions_motor_1)
\end{python}

This is repeated for the next three motors, creating an array with shape (4, 16). Each motor can be selected by choosing one of the larger arrays, and the direction is changed by reversing the order in which the bit-arrays are outputted. \\
Half-stepping involves powering two phases of the motor simultaneously in between each normal 'full' step, and decreases the angle moved in each step by a factor of two. This is done by using the following instructions:  
\begin{python}
states = [[1,0,0,0],[1,1,0,0],[0,1,0,0],[0,1,1,0],[0,0,1,0],[0,0,1,1],[0,0,0,1],[1,0,0,1]]
\end{python}

One can then define functions to allow the number of steps and the required direction to be input.
\begin{python}
def oneStep(motorNum, direction): 
    if direction==1:  
        for bits in instructions[motorNum]:  
            for bit in bits:             
                GPIO.output(DATA,int(bit))
                pulseClock() # push bits into storage
            pulseLatch()     # push stored bis to output pins
    elif direction==0:
        for bits in reversed(instructions[motorNum]): 
            for bit in bits:            
                GPIO.output(DATA, bit)
                pulseClock() 
            pulseLatch()    
def NSteps(nsteps, motorNum, direction):
    for n in range(nsteps):
        oneStep(motorNum, direction) 
    for bit in np.zeros(16): # Reset all motor phases to LOW 
        GPIO.output(DATA, bit)
        pulseClock() 
    pulseLatch()    
\end{python}

In the above code, each step is defined as four phases in full-stepping mode. To be able to access individual phases in either direction, the code must be able to track the number of steps taken by each motor, and in which direction.
\begin{python}
counters = [[1,0],[2,0],[3,0],[4,0]] # (Motor, NumSteps)
def oneStep(motor,direction):
        if direction==1:
            var = (counters[motor][1])%len(states) 
            bits = instructions[motor][var] 
            for bit in bits:    
                GPIO.output(DATA,bit)
                pulseClock() 
            pulseLatch()  
            counters[motor][1] += 1
        elif direction==0:
            var = (counters[motor][1])%len(states) 
            bits = instructions[motor][var-1] 
            for bit in bits:    
                GPIO.output(DATA,bit)
                pulseClock() 
            pulseLatch()  
            counters[motor][1] -= 1
\end{python}

\section{Interfacing with M-LOOP} 
M-LOOP operates by reading a text file, `exp-output.txt', containing a `cost' value, then using machine-learning algorithms to predict parameters which will minimise this cost. It then creates a text file, `exp-input.txt', which is read by a script controlling the motors. The text file created by M-LOOP contains the number of steps to be turned by the motors. After executing the step given by the text file, a reading is taken from the sensor. The cost is defined as the negative of this value, and so minimising the cost is equivalent to maximising the reading by the sensor.
Reading the files is achieved as follows
\begin{python}
condition = True
while condition:
    start_time = time.time()
    try:    
        time.sleep(0.2)  
        fileName = 'exp_input.txt'
        f = open(fileName, "r") 
        string = f.read()  
        f.close() 
        os.remove(fileName) 
        exec(string)  
        if time.time() > start_time + 20:
            condition = False
    except Exception as exception:
        print(exception)
        continue
\end{python}
 
Running the M-LOOP script and the motor-controlling script in parallel allows the algorithms to continually learn to optimise the sensor reading by controlling the steps by the motors and therefore the pitch and yaw of the mirrors. 

\section{Code for Deep Learning}
The code for the deep learning architecture created by Baumeister \textit{et al.} \cite{Kutz18} can be found at:\\
 \url{https://github.com/thombau/UW_Seattle_1}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Wiring} \label{sec:Wiring}
%%%%%%%%%%%%%%% Wiring 1 %%%%%%%%%%%%%%%%%
\textbf{Instructions:} Connect the pins from left to right across each table.
\begin{table}[h]
\centering
\caption[Wiring - Raspberry Pi to Shift Register]{The wiring from the Raspberry Pi to the Shift Register} 
\begin{tabular}{ c | c | c }
\textbf{RPI Pins} & \textbf{SR(1,2) Pins (74HC595)} & \textbf{Meaning} \\
 \hline
 17 (3V3) & 16 (VCC) & Power (3.3V) \\
 17 (3V3) & 10 (MR) & Needs to be HIGH\\
 34 (GND) & 8 (GND) & Ground \\
34 (GND) & 13 (OE) & Needs to be LOW \\
35 (GPIO 19) & 12 (STCP) & Latch \\
37 (GPIO 26) & 11 (SHCP) & Clock \\
33 (GPIO 13) & 14 (DS) & Data (\textit{specific to SR1 only})
\end{tabular}
\label{tab:Pi to SR}
\end{table}
%%%%%%%%%%%%%%% Wiring 2 %%%%%%%%%%%%%%%%%
\begin{table}[H]
\centering
\caption[Wiring - Shift Register 1 to Shift Register 2]{The wiring from the first shift register (SR1) to the second shift register (SR2) (both 74HC595).} 
\begin{tabular}{ c | c | c }
\textbf{SR1 Pins} & \textbf{SR2 Pins} & \textbf{Meaning} \\
 \hline
9 (Q7' or QH) & 14 (DS) & Output data of SR1 to Input data on SR2 \\
\end{tabular}
\label{tab:SR1 to SR2}
\end{table}

\normalsize \textit{Note: Connect Latch and Clock from SR1 to SR2 in parallel.}
%%%%%%%%%%%%%%% Wiring 3 %%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%% Wiring 4 %%%%%%%%%%%%%%%%%
\begin{table}[h]
\centering
\caption[Wiring - Driver 1 (L298N) to Shift Register 1]{The wiring from Driver 1 (Motor 1) to Shift Register 1 (74HC595)} 
\begin{tabular}{ c | c | c }
\large \textbf{Driver 1} & \large \textbf{SR1 Pins} & \large \textbf{Meaning} \\
 \hline
IN1 & 15 (Q0) & Coil 1 (Motor) \\
IN2 & 1 (Q1) & Coil 2 (Motor)\\
IN3 & 2 (Q2) & Coil 3 (Motor) \\
IN4 & 3 (Q3) & Coil 4 (Motor) \\
+ &  & +5 V Supply\\
- &  & 0 V Ground \\
\end{tabular}
\label{tab:Driver1 to SR1}
\end{table}
%%%%%%%%%%%%%%% Wiring 5 %%%%%%%%%%%%%%%%%
\begin{table}[H]
\centering
\caption[Wiring - Driver 2 (L298N) to Shift Register 1]{The wiring from Driver 2 (Motor 2) to Shift Register 1 (74HC595)} 
\begin{tabular}{ c | c | c }
\large \textbf{Driver 2} & \large \textbf{SR1 Pins} & \large \textbf{Meaning} \\
 \hline
IN1 & 4 (Q4) & Coil 1 (Motor) \\
IN2 & 5 (Q5) & Coil 2 (Motor)\\
IN3 & 6 (Q6) & Coil 3 (Motor) \\
IN4 & 7 (Q7) & Coil 4 (Motor) \\
+ &  & +5 V Supply\\
- &  & 0 V Ground \\
\end{tabular}
\label{tab:Driver2 to SR1}
\end{table}
\normalsize \textit{Note: Driver 3 and Driver 4 are to be connected to SR2 in the same configuration that Driver 1 and Driver 2 are connected to SR2.}
%%%%%%%%%%%%%%% Wiring 5 %%%%%%%%%%%%%%%%%
\begin{table}[h]
\centering
\caption[Wiring - ADC]{Additional wiring from the Analog-to-Digital Converter} 
\begin{tabular}{ c | c | c }
\large \textbf{ADC (ADS1115)} & \large \textbf{Other} & \large \textbf{Meaning} \\
 \hline
ADDR & GND & Address (if LOW, defaults to 0x48) \\
A0 & PD output (+5 V) & Analog Input Pin 0 (A0 chosen arbitrarily)
\end{tabular}
\label{tab:ADC Wiring}
\end{table}



\normalsize Similar diagrams for the pins of the shift registers can easily be found online.



%%%%%%%%%%%%% Photon counting %%%%%%%%%%%%
%\chapter{Photon Counting Investigation} \label{chap:proposed}
%This section details an investigation into the ability of M-LOOP to optimise the alignment of beams dominated by Poisson noise, given an additional week of experimental time. \\
 
%The ability of M-LOOP to converge on optimal parameters would be investigated for a range of values of SNR, where for Poisson-noise-dominated systems the SNR is given by $\sqrt{M}$. The SNR would be varied by changing the total optical density of the NDFs, or by using a variable iris.\\

%In order to assess M-LOOP's ability to converge on optimal parameters (and therefore its ability to align the beam), a measure of the rate of convergence for a given SNR is required. Similarly to the definition of the rise-time in electronics, it was decided that the number of machine-learning iterations required to reach 90\% of the final correlation length value would be taken as a measure of the rate of convergence \cite{vodovozov2010introduction}. This number of iterations would be plotted against the SNR, and it is expected that the results would show that the algorithm performs better as the SNR increases, based on the results of optimisation at low beam powers outlined in Section \ref{subsubsec:Results:Decreasing}. 
%This could be combined with the time taken by the algorithm at each value of SNR to provide a metric by which to compare human performance.\\


%\begin{comment}
%\begin{figure}[h]
 % \centering
  %\begin{minipage}[b]{0.45\textwidth}
   % \includegraphics[width=\textwidth]{figures/Photon_counter.pdf}
%\caption[Photograph - Photon Counter]{The SPCM-AQRH photon-counting device. Details can be found in Appendix \ref{chap:Parts}.\newline}
%\label{fig:Photon_counter}
%  \end{minipage}
%%  \hfill
 % \begin{minipage}[b]{0.45\textwidth}
  %  \includegraphics[width=\textwidth]{figures/Sensl_timing_module.pdf}
%\caption[Photograph - Timing Module]{The HRM-TDC module used to record the time of the incoming photons. Details can be found in Appendix \ref{chap:Parts}.}
%\label{fig:Timing_module}
 % \end{minipage}
%\end{figure}
%\end{comment}

\section{Continuous Auto-Optimisation} \label{chap:ContinuousAutoOpt}
%What industries use PID? All?
Continual optimisation of a system is employed to correct for variations in a signal, for example due to mechanical creep, unstable dynamics, or thermal and sensor fluctuations.
One of the simplest and most common types of feedback control method is the proportional-integral-derivative (PID) controller \cite{bansal2012pid}, which often requires parameters to be set manually.
However, after some time, the set control-parameters may no longer match the system and the signal will be forced to oscillate.
A system which could change control parameters responsively would be a more effective method of control, and the potential of M-LOOP to act as such a system was investigated.\\

Whilst M-LOOP was not designed for continual optimisation, modifications to the software can be made which allow it to function more as an `optimiser' than a `scientist'. By setting the coefficient of the covariance matrix in the biased cost, $B_C$, close to zero, it is possible to force M-LOOP to prioritise finding parameters which minimise the cost (see Section \ref{subsubsec:MLOOPOptimisation}). This was paired with restricting the algorithm's search range and trust-region (see Section \ref{subsubsec:Overview}), such that if the system is close to the optimum, it would not stray far from it.\\
 
As stated in Section \ref{subsubsec:Methods:ML:General}, the algorithm completes one optimisation run and terminates only once one of several user-defined halting conditions are met. 
One strategy to achieve continual optimisation is to let the algorithm run indefinitely, assuming that the model will converge on a correlation length and remain there, predicting optimal parameters at each iteration and keeping the beam in optimal alignment. This can be achieved by either setting the maximum number of iterations to a very large number, or to set the cost at which the algorithm will terminate to a value which is impossible to achieve.
This strategy fails due to the increasing computational time taken at each iteration (see Section \ref{subsubsec:Methods:ML:General}). The time taken becomes noticeably long around four-hundred iterations with each iteration taking upwards of thirty seconds, and therefore this method of continuous optimisation is infeasible.\\

Another strategy is to set the maximum number of iterations such that the model converges on optimal parameters and then shuts down, repeating this process periodically. However, as successive optimisations are independent of each other, M-LOOP is unable to learn from previous optimisations and must rediscover the optimal parameters at each run. The amount of time to convergence is also significant, taking just over five minutes using 150 maximum iterations. When the number of iterations per optimisation run was decreased below 100, it was found that the final beam intensity varied by up to 10\% of the maximum reading.
Given that M-LOOP shuts down between runs, there is an inevitable trade-off between the number of iterations per run (and therefore the computational time) and the accuracy of the optimised parameters.\\

A third strategy tested was to use a Gaussian process to discover optimal parameters, then use a classical optimisation algorithm (Nelder-Mead via M-LOOP) to maintain the alignment. However, the signal was found to drift over time and this method was not pursued any further. 
The Allan Deviation was used to measure the stability of the signal over time and quantify the level of noise for each method described above \cite{czerwinski2009quantifying, el2007analysis}. However, due to the intensity fluctuations present in the signal, this did not return useful results.
M-LOOP is slower and less accurate than currently-available technology for continuous alignment (Table \ref{tab:Thorlabs}), and should not be used for this purpose in its current form. \\

%%%%%%%%%%%%% Equation Derivation %%%%%%%%%%%%%%%%%%
\chapter{Equation Derivation} 
\begin{figure}
  \centering
  \begin{minipage}[b]{0.45\textwidth}
    \includegraphics[width=\textwidth]{figures/NewEquation-cropped.pdf} 
\caption[]{A ray diagram showing a laser beam (red) incident on a mirror and focussed by a lens with focal length $f$ onto the focal plane. The finely dotted line indicates the axis through the centre of the mirror. \newline \newline \newline \newline \newline \newline \newline}
 \label{fig:2D schematic-1}
  \end{minipage}
  \hfill
  \begin{minipage}[b]{0.45\textwidth}
    \includegraphics[width=\textwidth]{figures/NewEquation2-cropped.pdf}
\caption[]{A ray diagram showing a laser beam (red) incident on a mirror and focused by a lens with focal length $f$ onto the focal plane. The distance from the pivot of the mirror-mount to the point of action of the stepper motor is labelled $L$, and the mirror is displaced by a distance $z$ at the motor. The motor causes the mirror to rotate by an angle $\theta$ and therefore the beam is also displaced by $\theta$, causing a linear displacement from the origin of $\Delta y$ after focussing by the lens. The finely dotted lines indicate the axes through the centre of the mirror before and after the mirror has rotated by $\theta$. }
\label{fig:2D schematic-2}
  \end{minipage}

\end{figure}
 
\begin{figure}
\centering
\includegraphics[width=0.7\textwidth]{figures/3D NewEquation-cropped.pdf} 
\caption[Equation Schematic 3D]{The schematic describes the path of a laser beam onto the mouth of an optical fibre. Schematic shows the path the beam (red) from a laser (1), incident on two mirrors (2,3) and being focused by a lens (4) onto the focal plane (5). The second mirror (3) is tilted by a polar angle $\theta$ (pitch) and azimuthal angle $\phi$ (yaw), and the effect of the lens is to convert this angular displacement into a linear displacement in the focal plane. The beam is displaced by $\Delta x$ in the $x$ axis and by $\Delta y$ in the $y$ axis}
\label{fig:3D schematic}
\end{figure} 
 
To convert the number of steps turned by the stepper motor into a corresponding distance moved across the mouth of a photodiode or an optical fibre, we must define several things:\\
The reciprocal of the threads-per-inch (tpi) of a screw is its pitch, and is synonymous with the distance travelled by the screw per revolution, and is given the symbol $p$.
The number of steps per revolution of the stepper motor is given the symbol $s$.
The number of steps by the motor is given the symbol $n$.
The distance travelled by the screw is given the symbol $z$.
The distance from the point of action of the leadscrew to the pivot is given the symbol $L$.
The angle moved by the mirror mount is given the symbol $\theta$. \\


The distance $z$ is calculated using the following:\\
\begin{equation}
z = \frac{\text{distance}}{\text{revolution}} \frac{\text{revolutions}}{\text{step}} \, \text{number} \, \text{of} \, \text{steps} \, ,
\end{equation}

which, using the defined symbols, is:

\begin{equation}
z = \frac{p \, n}{s} \, .
\end{equation}


By approximating the triangle formed by the mirror mount before and after being acted upon by the leadscrew as a right-angled triangle, the angle $\theta$ is given by
\begin{equation}
\tan(\theta) = \frac{z}{L} \, ,
\end{equation}

and for small $z/L$ this becomes

\begin{equation}
\theta \approx \frac{z}{L} \, .
\end{equation}


When the mirror knob is rotated by the motor, the mirror mount pitches forwards by an angle $\theta$. The effect of the lens is to turn angular displacements into linear displacements in the focal plane, given by 

\begin{equation}
\Delta y = f \theta \,  ,
\end{equation}

where $f$ is the focal length of the lens and $\Delta y$ is the linear displacement in the focal plane. Substituting in for $\theta$ and then $z$ we get

\begin{equation}
\Delta y = f \frac{pn}{Ls} \, .
\label{eqn:ConversionEquation}
\end{equation}

Using a mirror mount with control over two degrees of freedom,  it is possible to convert the pitch and the yaw, given by $\theta$ and $\phi$ respectively, into linear displacements $\Delta y$ and $\Delta x$ in the focal plane respectively. This is shown schematically in Fig. \ref{fig:2D schematic-1}, \ref{fig:2D schematic-2} and \ref{fig:3D schematic}. 


The numerical values for all quantities are:\\
%$R$ = 36 $\pm$ 1 mm\\
$L$ = 35 $\pm$ 1 mm\\
LIOP-TEC mounts: $p$ = $\frac{1}{170}$\\
Thorlabs mount: $p$ = $\frac{1}{80}$\\
28BY-J48 motor: $s$ = 64 (full-stepping mode) - \textit{Note:} this motor also includes a gear reduction of 64.\\
NEMA-17 motor: $s$ = 200 (full-stepping mode)\\

\chapter{Additional Graphs} \label{chap:Additional Graphs}
%% ratio R of intensities
\begin{figure}[H]
  \centering
    \includegraphics[width=0.8\textwidth]{figures/Ratio_plot_cos(2A).pdf}
    \caption[Ratio of Intensities]{The ratio of the difference and sum of the beam intensities, $R_I$, plotted over twenty-four hours at ten-second intervals. $R_I$ varies very little over twenty-four hours, suggesting that there is little, if any, polarisation noise present(?-see later paragraphs).}
\label{fig:Ratio_full}
\end{figure}

%% sum S of intensities
\begin{figure}[H]
  \centering
    \includegraphics[width=0.8\textwidth]{figures/Intensity_plot_I0.pdf}
    \caption[Sum of Intensities]{The sum of the intensities of each beam arm, $S_I$, plotted over twenty-four hours at ten-second intervals. The sum is not constant, and varies by 150 mV over twenty-four hours and therefore there must be fluctuations in the intensity of the laser, i.e. $I_1$ is not constant. There are faster oscillations in $S_I$ which are explained by over-driving of the laser power supply.}
\label{fig:Sum_full}
\end{figure}


%\end{appendices}
%The analog-to-digital converter used in this project is the ADS1115 by Adafruit, who have written pre-made libraries to read data from their chips. To communicate with the chip it is necessary to download the library ‘Adafruit-CircuitPython-ADS1x15’ from their GitHub, and add the library to the path.

\section{\label{sec:SRs}Operating the shift registers}

\section{\label{sec:Int_with_MLOOP}Interfacing with M-LOOP}












==> REFERENCES.tex <==
\usepackage{url}

@PREAMBLE{
 "\providecommand{\noopsort}[1]{}" 
 # "\providecommand{\singleletter}[1]{#1}%" 
}
@incollection{ ISI:000412476200021,
Author = {Goodfellow, I and Bengio, Y. and Courville, A.},
Book-Author = {{Goodfellow, I
   Bengio, Y
   Courville, A}},
Title = {{Deep Learning}},
Booktitle = {{Deep Learning}},
Series = {{Adaptive Computation and Machine Learning}},
publisher = {{MIT press}},
Year = {{2016}},
%Pages = {{1-775}},
ISBN = {{978-0-262-03561-3}},
Unique-ID = {{ISI:000412476200021}},
}

@MISC{MLOOP,
   author       = {M. R. Hush}, 
   howpublished = "\url{https://m-loop.readthedocs.io/en/latest/api/mloop.html}",
   year         = {2016},
}



@incollection{ Murphy12,
Author = {{Murphy, K P}},
Book-Author = {{Murphy, K P}},
Title = {{Machine Learning: A Probabilistic Perspective}},
Booktitle = {{Machine Learning: A Probabilistic Perspective}},
Series = {{Adaptive Computation and Machine Learning}},
publisher = {{MIT press}},
Year = {{2012}},
%Pages = {{1-775}},
ISBN = {{9780262018029}}},
%Unique-ID = {{ISI:000412476200021}},
}

@ARTICLE{Judson92,
   author       = "R. S. Judson and H. Rabitz",
   year         = "1992",
   journal      = "Physical Review Letters",
   volume       = "68",
   pages        = "1500",
}


@ARTICLE{Hush16,
   author       = {Wigley, P. B. and Everitt, P. J. and van den Hengel, A. and Bastian, J.
   W. and Sooriyabandara, M. A. and McDonald, G. D. and Hardman, K. S. and
   Quinlivan, C. D. and Manju, P. and Kuhn, C. C. N. and Petersen, I. R.
   and Luiten, A. N. and Hope, J. J. and Robins, N. P. and Hush, M. R.},
   journal = "Scientific Reports",
   pages = "25890",
   publisher = "Nature Publishing Group",
   title = "Fast machine-learning online optimization of ultra-cold-atom experiments",
   volume = "6",
   year = "2016"
}
@inproceedings{Kutz:14,
author = {J. Nathan Kutz and Xing Fu and Steven Brunton},
booktitle = {Advanced Photonics},
journal = {Advanced Photonics},
keywords = {Lasers, fiber; Mode-locked lasers; Ultrafast lasers; Birefringence; Fiber lasers; Mode locking; Nonlinear optical fibers; Optical components; Optical systems},
%pages = {NTu4A.7},
publisher = {Optical Society of America},
title = {Self-tuning fiber lasers: machine learning applied to optical systems},
year = {2014},
url = {http://www.osapublishing.org/abstract.cfm?URI=NP-2014-NTu4A.7},
doi = {10.1364/NP.2014.NTu4A.7},
abstract = {We demonstrate that machine learning with adaptive control is capable of producing an efficient and optimal self-tuning algorithm for mode-locked fiber lasers. The methods can generalized to a variety of optical systems.},
}


@ARTICLE{Grelu16,
   author       = "Andral, U and Buguet, J and Fodil, R Si and Amrani, F and Billard, F and Hertz, E and Grelu, Ph", 
   year         = "2016", 
   journal      = "Journal of the Optical Society of America B", 
   volume       = "33", 
   pages        = "825",
}
@ARTICLE{Kutz18,
   author       = "Baumeister, T and Brunton, S. L. and Kutz, J. N.",
   year         = "2018", 
   journal      = "Journal of the Optical Society of America B", 
   volume       = "35", 
   pages        = "617",
}
@ARTICLE{Gong16,
   author       = "Zhang, Y and Wu, C and Song, Y and Si, K and Zheng, Y and Hu, L and Chen, J and Tang, L and Gong, W", 
   year         = "2016", 
   journal      = "Optics Express", 
   volume       = "27", 
   pages        = "16871",
}
@ARTICLE{Briegel18,
   author       = "Melnikov, A. A. and Nautrup,  H. P. and Krenn, M. and Dunjko, V. and Tiersch, M. and Zeilinger,  A. and Briegel, H. J.", 
   year         = "2018", 
   journal      = "Proceedings of the National Academy of Sciences", 
   volume       = "27", 
   pages        = "16871",
}

@BOOK{Adams12,
   author       = {B. Adams}, 
   year         = 2012, 
   title      = {Nonlinear Optics, Quantum Optics, and Ultrafast Phenomena with
X-Rays: Physics with X-Ray Free-Electron Lasers.}, 
    publisher    = {Springer US}
}
@ARTICLE{Cooper20,
   author       = "Burger, B. and Maffettone, P. and Gusev, V. and Aitchison, C. and Bai, Y. and Xiaoyan, W. and Sprick, R. S. and Cooper, A. I.", 
   year         = "2020", 
   journal      = "Nature", 
   volume       = "583", 
}

@article{Whiting_2017,
   title={Single-Photon Interference due to Motion in an Atomic Collective Excitation},
   volume={118},
   number={25},
   journal={Physical Review Letters},
   publisher={American Physical Society (APS)},
   author={Whiting, D. J. and Šibalić, N. and Keaveney, J. and Adams, C. S. and Hughes, I. G.},
   year={2017},
   month={Jun}
}

@book{f2f,
    author    = "C. S. Adams and I. G. Hughes",
    title     = "Optics f2f - From Fourier to Fresnel",
    year      = "2019",
    publisher = "Oxford University Press",
    address   = "Oxford, UK"
}

@book{errors,
    author    = "I. G. Hughes and T. P. A. Hase",
    title     = "Measurements and their Uncertainties",
    year      = "2010",
    publisher = "Oxford University Press",
    address   = "Oxford, UK"
}

@article{doi:10.1063/1.5025729,
author = {Nemchick,Deacon J. and Drouin,Brian J. and Cich,Matthew J. and Crawford,Timothy and Tang,Adrian J. and Kim,Yanghyo and Reck,Theodore J. and Schlecht,Erich T. and Chang,M.-C. Frank and Virbila,Gabriel },
title = {A 90-102 GHz CMOS based pulsed Fourier transform spectrometer: New approaches for in situ chemical detection and millimeter-wave cavity-based molecular spectroscopy},
journal = {Review of Scientific Instruments},
volume = {89},
number = {7},
pages = {073109},
year = {2018},
}

@article{doi:10.1063/1.4986044,
author = {Benítez,Alfredo  and Santiago,Ulises  and Sanchez,John E.  and Ponce,Arturo },
title = {Design of a cathodoluminescence image generator using a Raspberry Pi coupled to a scanning electron microscope},
journal = {Review of Scientific Instruments},
volume = {89},
number = {1},
pages = {013702},
year = {2018},

}

@article{doi:10.1063/1.5071447,
author = {Zapata-Farfan,Jennyfer  and Contreras-Martínez,Ramiro  and Rosete-Aguilar,Martha  and Garduño-Mejía,Jesús  and Castro-Marín,Pablo  and Rodríguez-Herrera,Oscar G.  and Bruce,Neil C.  and Ordóñez-Pérez,Mitzi  and Qureshi,Naser  and Ascanio,Gabriel },
title = {Low-energy/pulse response and high-resolution-CMOS camera for spatiotemporal femtosecond laser pulses characterization @ 1.55 μm},
journal = {Review of Scientific Instruments},
volume = {90},
number = {4},
pages = {045116},
year = {2019},

}

@article{doi:10.1063/1.5022973,
author = {Keaveney,James },
title = {Automated translating beam profiler for in situ laser beam spot-size and focal position measurements},
journal = {Review of Scientific Instruments},
volume = {89},
number = {3},
pages = {035114},
year = {2018},

}
@article{doi:10.1063/1.4941068,
author = {Sharkey,James P.  and Foo,Darryl C. W.  and Kabla,Alexandre  and Baumberg,Jeremy J.  and Bowman,Richard W. },
title = {A one-piece 3D printed flexure translation stage for open-source microscopy},
journal = {Review of Scientific Instruments},
volume = {87},
number = {2},
pages = {025104},
year = {2016},
}


@article{doi:10.1063/1.4972255,
author = {Clayburn,N. B.  and Trantham,K. W.  and Dunn,M.  and Gay,T. J. },
title = {Method for monitoring GaAs photocathode heat cleaning temperature},
journal = {Review of Scientific Instruments},
volume = {87},
number = {12},
pages = {124903},
year = {2016},
}

@article{doi:10.1063/1.5066062,
author = {Cremers,Theo  and Janssen,Niek  and Sweers,Edwin  and van de Meerakker,Sebastiaan Y. T. },
title = {Design and construction of a multistage Zeeman decelerator for crossed molecular beams scattering experiments},
journal = {Review of Scientific Instruments},
volume = {90},
number = {1},
pages = {013104},

year = {2019},
}

@article{PhysRevA.79.033814,
  title = {Four-wave mixing in the diamond configuration in an atomic vapor},
  author = {Willis, R. T. and Becerra, F. E. and Orozco, L. A. and Rolston, S. L.},
  journal = {Phys. Rev. A},
  volume = {79},
  issue = {3},
  pages = {033814},
  numpages = {6},
  year = {2009},
  month = {Mar},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.79.033814},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.79.033814}
}

@article{ ISI:000286728700022,
Author = {Willis, R. T. and Becerra, F. E. and Orozco, L. A. and Rolston, S. L.},
Title = {Correlated photon pairs generated from a warm atomic ensemble},
Journal = {Phys. Rev. A},
Year = {2010},
Volume = {82},
Number = {5},
Month = {{NOV 30}},
pages = {053842},
}


@article{Willis:11,
author = {R. T. Willis and F. E. Becerra and L. A. Orozco and S. L. Rolston},
journal = {Opt. Express},
keywords = {Multiphoton processes; Photon statistics; Quantum information and processing ; Atomic ensembles; Parametric down conversion; Photon polarization; Photon statistics; Photons; Quantum cryptography},
number = {15},
pages = {14632--14641},
publisher = {OSA},
title = {Photon statistics and polarization correlations at telecommunications wavelengths from a warm atomic ensemble},
volume = {19},
month = {Jul},
year = {2011},
url = {http://www.opticsexpress.org/abstract.cfm?URI=oe-19-15-14632},
doi = {10.1364/OE.19.014632},
abstract = {We present measurements of the polarization correlation and photon statistics of photon pairs that emerge from a laser-pumped warm rubidium vapor cell. The photon pairs occur at 780 nm and 1367 nm and are polarization entangled. We measure the autocorrelation of each of the generated fields as well as the cross-correlation function, and observe a strong violation of the two-beam Cauchy-Schwartz inequality. We evaluate the performance of the system as source of heralded single photons at a telecommunication wavelength. We measure the heralded autocorrelation and see that coincidences are suppressed by a factor of $\approx$ 20 from a Poissonian source at a generation rate of 1500 s{\textminus}1, a heralding efficiency of 10\%, and a narrow spectral width.},
}
@article{PhysRevLett.109.033601,
  title = {Tomography of a High-Purity Narrowband Photon from a Transient Atomic Collective Excitation},
  author = {MacRae, A. and Brannan, T. and Achal, R. and Lvovsky, A. I.},
  journal = {Phys. Rev. Lett.},
  volume = {109},
  issue = {3},
  pages = {033601},
  numpages = {4},
  year = {2012},
  month = {Jul},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.109.033601},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.109.033601}
}

@article{doi:10.1080/09500340.2017.1377308,
author = {D. J. Whiting and Renju S. Mathew and J. Keaveney and C. S. Adams and I. G. Hughes},
title = {Four-wave mixing in a non-degenerate four-level diamond configuration in the hyperfine Paschen–Back regime},
journal = {Journal of Modern Optics},
volume = {65},
number = {5-6},
pages = {713-722},
year  = {2018},
publisher = {Taylor & Francis},
}


@article{PhysRevA.93.053821,
  title = {Coupling of four-wave mixing and Raman scattering by ground-state atomic coherence},
  author = {Parniak, Micha\l{} and Leszczy\ifmmode \acute{n}\else \'{n}\fi{}ski, Adam and Wasilewski, Wojciech},
  journal = {Phys. Rev. A},
  volume = {93},
  issue = {5},
  pages = {053821},
  numpages = {7},
  year = {2016},
  month = {May},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.93.053821},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.93.053821}
}
@article{Ding:12,
author = {Dong-Sheng Ding and Zhi-Yuan Zhou and Bao-Sen Shi and Xu-Bo Zou and Guang-Can Guo},
journal = {Opt. Express},
keywords = {Upconversion; Coherent optical effects; Nonlinear wave mixing ; Four wave mixing; Laser trapping; Near infrared radiation; Quantum communications; Raman scattering; Tunable diode lasers},
number = {10},
pages = {11433--11444},
publisher = {OSA},
title = {Generation of non-classical correlated photon pairs via a ladder-type atomic configuration: theory and experiment},
volume = {20},
month = {May},
year = {2012},
url = {http://www.opticsexpress.org/abstract.cfm?URI=oe-20-10-11433},
doi = {10.1364/OE.20.011433},
abstract = {We experimentally generate a non-classical correlated two-color photon pair at 780 and 1529.4 nm in a ladder-type configuration using a hot 85Rb atomic vapor with the production rate of ~107/s. The non-classical correlation between these two photons is demonstrated by strong violation of Cauchy-Schwarz inequality by the factor R $=$ 48 {\textpm} 12. Besides, we experimentally investigate the relations between the correlation and some important experimental parameters such as the single-photon detuning, the powers of pumps. We also make a theoretical analysis in detail and the theoretical predictions are in reasonable agreement with our experimental results.},
}
@article{Lee:16,
author = {Yoon-Seok Lee and Sang Min Lee and Heonoh Kim and Han Seb Moon},
journal = {Opt. Express},
keywords = {Quantum optics; Coherent optical effects; Nonlinear wave mixing ; Atomic ensembles; Photon correlations; Quantum key distribution; Quantum light sources; Quantum optics; Quantum teleportation},
number = {24},
pages = {28083--28091},
publisher = {OSA},
title = {Highly bright photon-pair generation in Doppler-broadened ladder-type atomic system},
volume = {24},
month = {Nov},
year = {2016},
url = {http://www.opticsexpress.org/abstract.cfm?URI=oe-24-24-28083},
doi = {10.1364/OE.24.028083},
abstract = {We report a bright photon-pair source with a coincidence counting rate per input power (cps/mW) of tens of thousands, obtained via spontaneous four-wave mixing from a Doppler-broadened atomic ensemble of the 5S1/2\&\#x2212;5P3/2\&\#x2212;5D5/2 transition of 87Rb. The photon-pair generation rate is enhanced by the two-photon coherence contributions from almost all the atomic velocity groups in the Doppler-broadened ladder-type atomic system. We obtained the violation of the Cauchy-Schwarz inequality by a factor of 2370 \&\#x00B1; 150. We believe that our scheme for highly bright paired photons is important as a useful quantum light source for quantum entanglement swapping between completely autonomous sources.},
}

@article{PhysRevA.93.043854,
  title = {Direct measurement of excited-state dipole matrix elements using electromagnetically induced transparency in the hyperfine Paschen-Back regime},
  author = {Whiting, Daniel J. and Keaveney, James and Adams, Charles S. and Hughes, Ifan G.},
  journal = {Phys. Rev. A},
  volume = {93},
  issue = {4},
  pages = {043854},
  numpages = {7},
  year = {2016},
  month = {Apr},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.93.043854},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.93.043854}
}
@article{Jeong:20,
author = {Taek Jeong and Han Seb Moon},
journal = {Opt. Express},
keywords = {Atomic ensembles; Cold atoms; Photon correlations; Quantum communications; Spectral properties; Tunable diode lasers},
number = {3},
pages = {3985--3994},
publisher = {OSA},
title = {Temporal- and spectral-property measurements of narrowband photon pairs from warm double-\&\#x039B;-type atomic ensemble},
volume = {28},
month = {Feb},
year = {2020},
url = {http://www.opticsexpress.org/abstract.cfm?URI=oe-28-3-3985},
doi = {10.1364/OE.385896},
abstract = {We investigate the temporal and spectral properties of narrowband photon pairs from a double-\&\#x039B;-type atomic system of a warm 87Rb atomic ensemble. The temporal properties of the narrowband photons are investigated by measuring their auto-correlation and cross-correlation functions. The spectral measurement of the photon pair is obtained by applying the stimulated emission method. We show that the biphoton spectral waveform with a spectral width of \&\#x223C;6\&\#x2005;MHz corresponds to the biphoton temporal waveform with a temporal width of \&\#x223C;26\&\#x2005;ns. We believe that our results can contribute to the characterization of narrowband photons generated from atomic ensembles and aid in the development of new photonic quantum states generated from atomic systems.},
}

@article{PhysRevA.100.033818,
  title = {Stimulated measurement of spontaneous four-wave mixing from a warm atomic ensemble},
  author = {Jeong, Taek and Park, Jiho and Moon, Han Seb},
  journal = {Phys. Rev. A},
  volume = {100},
  issue = {3},
  pages = {033818},
  numpages = {6},
  year = {2019},
  month = {Sep},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.100.033818},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.100.033818}
}

@article{Wang:s,
author = {Chengyuan Wang and Chung-Hyun Lee and Yoon-Ho Kim},
journal = {Opt. Express},
keywords = {Ghost imaging; Photonic entanglement; Quantum communications; Quantum imaging; Quantum information processing; Quantum key distribution},
number = {24},
pages = {34611--34617},
publisher = {OSA},
title = {Generation and characterization of position-momentum entangled photon pairs in a hot atomic gas cell},
volume = {27},
month = {Nov},
year = {2019} ,
}

@article{PhysRevLett.122.143601,
  title = {Polarization-Entangled Photons from a Warm Atomic Ensemble Using a Sagnac Interferometer},
  author = {Park, Jiho and Kim, Heonoh and Moon, Han Seb},
  journal = {Phys. Rev. Lett.},
  volume = {122},
  issue = {14},
  pages = {143601},
  numpages = {6},
  year = {2019},
  month = {Apr},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.122.143601},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.122.143601}
}

@article{Mika_2020,
	doi = {10.1088/1361-6455/ab8717},
	url = {https://doi.org/10.1088\%2F1361-6455\%2Fab8717},
	year = 2020,
	month = {jun},
	publisher = {{IOP} Publishing},
	volume = {53},
	number = {14},
	pages = {145501},
	author = {J Mika and L Slodi{\v{c}}ka},
	title = {High nonclassical correlations of large-bandwidth photon pairs generated in warm atomic vapor},
	journal = {Journal of Physics B: Atomic, Molecular and Optical Physics},
	abstract = {Generation of nonclassical light suitable for interaction with atoms corresponds to a crucial goal pursued across the broad quantum optics community. We present the generation of nonclassical photon pairs using the process of spontaneous four-wave mixing in warm atomic vapor with an unprecedentedly high degree of nonclassical photon correlations. We show how the unique combination of excitation of atoms in the proximity of the vapor cell viewport, single excitation laser beam, double-Λ energy level scheme, auxiliary optical pumping, and particular optical filtering setups, allow for the spectral bandwidth of generated nonclassical light fields of up to 560 ± 20 MHz and low two-photon noise. We provide a quantitative analysis of particular noise mechanisms which set technological and fundamental limits on the observable photon correlations. The overall technological simplicity of the presented scheme together with the availability of spectrally matched quantum memories implementable with warm atomic vapors promises the feasibility of realization of GHz bandwidth on-demand nonclassical light sources and efficient quantum communication nodes.}
}

@misc{burt2019rates,
    title={Rates of Convergence for Sparse Variational Gaussian Process Regression},
    author={David R. Burt and Carl E. Rasmussen and Mark van der Wilk},
    year={2019},
    eprint={1903.03571},
    archivePrefix={arXiv}
}
